Bregman Graph Neural Network

Numerous recent research on graph neural networks (GNNs) has focused on formulating GNN architectures as an optimization problem with the smoothness assumption. However, in node classification tasks, the smoothing effect induced by GNNs tends to assimilate representations and over-homogenize labels of connected nodes, leading to adverse effects such as over-smoothing and misclassification. In this paper, we propose a novel bilevel optimization framework for GNNs inspired by the notion of Bregman distance. We demonstrate that the GNN layer proposed accordingly can effectively mitigate the over-smoothing issue by introducing a mechanism reminiscent of the "skip connection". We validate our theoretical results through comprehensive empirical studies in which Bregman-enhanced GNNs outperform their original counterparts in both homophilic and heterophilic graphs. Furthermore, our experiments also show that Bregman GNNs can produce more robust learning accuracy even when the number of layers is high, suggesting the effectiveness of the proposed method in alleviating the over-smoothing issue.

==> Old/full_refs.tex <==
@inproceedings{frecon2022bregman,
  title={Bregman Neural Networks},
  author={Frecon, J. and Gasso, G. and Pontil, M. and Salzo, S.},
  booktitle={ICML},
  pages={6779--6792},
  year={2022}, 
}
@inproceedings{yang2016revisiting,
  title={Revisiting semi-supervised learning with graph embeddings},
  author={Yang, Zhilin and Cohen, William and Salakhudinov, Ruslan},
  booktitle={ICML},
  pages={40--48},
  year={2016}, 
}
@article{shchur2018pitfalls,
  title={Pitfalls of graph neural network evaluation},
  author={Shchur, Oleksandr and Mumme, Maximilian and Bojchevski, Aleksandar and G{\"u}nnemann, Stephan},
  journal={arXiv preprint arXiv:1811.05868},
  year={2018}
}
@inproceedings{mcauley2015image,
  title={Image-based recommendations on styles and substitutes},
  author={McAuley, Julian and Targett, Christopher and Shi, Qinfeng and Van Den Hengel, Anton},
  booktitle={Proceedings of the 38th International ACM SIGIR Conference on Research and Development in Information Retrieval},
  pages={43--52},
  year={2015}
}
@inproceedings{defferrard2016convolutional,
  title={Convolutional neural networks on graphs with fast localized spectral filtering},
  author={Defferrard, Micha{\"e}l and Bresson, Xavier and Vandergheynst, Pierre},
  booktitle={NeurIPS}, 
  year={2016}, 
}
@inproceedings{velivckovic2018graph,
  title={Graph attention networks},
  author={Veli{\v{c}}kovi{\'c}, Petar and Cucurull, Guillem and Casanova, Arantxa and Romero, Adriana and Lio, Pietro and Bengio, Yoshua},
  booktitle={ICLR},
  year={2018},
  doi={https://doi.org/10.17863/CAM.48429}
}
@inproceedings{xu2018how,
  author    = {Keyulu Xu and
               Weihua Hu and
               Jure Leskovec and
               Stefanie Jegelka},
  title     = {How Powerful are Graph Neural Networks?},
  booktitle = {ICLR}, 
  year      = {2019},
  url       = {https://openreview.net/forum?id=ryGs6iA5Km},
  timestamp = {Thu, 25 Jul 2019 13:03:15 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/XuHLJ19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{hamilton2017inductive,
  author    = {Hamilton, Will and Ying, Zhitao and Leskovec, Jure},
  title     = {Inductive representation learning on large graphs},
  booktitle = {NeurIPS}, 
  year      = {2019},
  url       = {https://openreview.net/forum?id=H1gL-2A9Ym},
  timestamp = {Thu, 25 Jul 2019 14:25:49 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/KlicperaBG19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{KlicperaBG19,
  author    = {Johannes Klicpera and
               Aleksandar Bojchevski and
               Stephan G{\"{u}}nnemann},
  title     = {Predict then Propagate: Graph Neural Networks meet Personalized PageRank},
  booktitle = {ICLR}, 
  year      = {2019},
  url       = {https://openreview.net/forum?id=H1gL-2A9Ym},
  timestamp = {Thu, 25 Jul 2019 14:25:49 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/KlicperaBG19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{kipf2017semisupervised,
  author    = {Thomas N. Kipf and
               Max Welling},
  title     = {Semi-Supervised Classification with Graph Convolutional Networks},
  booktitle = {ICLR},
  year      = {2017},
  url       = {https://openreview.net/forum?id=SJU4ayYgl},
  timestamp = {Thu, 25 Jul 2019 14:25:55 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/KipfW17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{xu2018representation,
  title={Representation learning on graphs with jumping knowledge networks},
  author={Xu, Keyulu and Li, Chengtao and Tian, Yonglong and Sonobe, Tomohiro and Kawarabayashi, Kenichi and Jegelka, Stefanie},
  booktitle={International Conference on Machine Learning},
  pages={5453--5462},
  year={2018},
  organization={PMLR}
}
@article{abs-1909-13021,
  title={Multi-scale attributed node embedding},
  author={Rozemberczki, Benedek and Allen, Carl and Sarkar, Rik},
  journal={Journal of Complex Networks},
  volume={9},
  number={2},
  pages={cnab014},
  year={2021},
  publisher={Oxford University Press}
} % tbd
@inproceedings{Pei2020Geom-GCN,
  title     = {{Geom-GCN}: Geometric Graph Convolutional Networks},
  author    = {Hongbin Pei and
               Bingzhe Wei and
               Kevin Chen{-}Chuan Chang and
               Yu Lei and
               Bo Yang},
  booktitle = {ICLR}, 
  year      = {2020},
  url       = {https://openreview.net/forum?id=S1e2agrFvS},
  timestamp = {Wed, 10 Feb 2021 11:28:14 +0100},
  biburl    = {https://dblp.org/rec/conf/iclr/PeiWCLY20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{Tang2009,
author = {Tang, Jie and Sun, Jimeng and Wang, Chi and Yang, Zi},
title = {Social Influence Analysis in Large-Scale Networks},
year = {2009},
isbn = {9781605584959},
publisher = {Association for Computing Machinery},
url = {https://doi.org/10.1145/1557019.1557108},
doi = {10.1145/1557019.1557108},
booktitle = {Proceedings of the 15th ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
pages = {807–816},
numpages = {10},
keywords = {social networks, topical analysis propagation, large-scale network, social influence analysis},
series = {KDD '09}
}
@inproceedings{Bruna2014,
  author       = {Joan Bruna and
                  Wojciech Zaremba and
                  Arthur Szlam and
                  Yann LeCun},
  title        = {Spectral Networks and Locally Connected Networks on Graphs},
  booktitle    = {International Conference on Learning Representations},
  year         = {2014},
  url          = {http://arxiv.org/abs/1312.6203},
}
@inproceedings{li2018adaptive,
  title={Adaptive graph convolutional neural networks},
  author={Li, Ruoyu and Wang, Sheng and Zhu, Feiyun and Huang, Junzhou},
  booktitle={AAAI},
  volume={32},
  number={1},
  year={2018}
}
@inproceedings{zhuang2018,
  title={Dual graph convolutional networks for graph-based semi-supervised classification},
  author={Zhuang, Chenyi and Ma, Qiang},
  booktitle={The WWW},
  pages={499--508},
  year={2018}
}
@inproceedings{
xu2018graph,
title={Graph Wavelet Neural Network},
author={Xu, Bingbing and Shen, Huawei and Cao, Qi and Qiu, Yunqi and Cheng, Xueqi},
booktitle={International Conference on Learning Representations},
year={2019},
url={https://openreview.net/forum?id=H1ewdiR5tQ},
}
@InProceedings{mixhop,
  title = 	 {{M}ix{H}op: Higher-Order Graph Convolutional Architectures via Sparsified Neighborhood Mixing},
  author =       {Abu-El-Haija, Sami and Perozzi, Bryan and Kapoor, Amol and Alipourfard, Nazanin and Lerman, Kristina and Harutyunyan, Hrayr and Steeg, Greg Ver and Galstyan, Aram},
  booktitle = 	 {Proceedings of the 36th International Conference on Machine Learning},
  pages = 	 {21--29},
  year = 	 {2019},
  volume = 	 {97},
  series = 	 {Proceedings of Machine Learning Research},
  publisher =    {PMLR},
  url = 	 {https://proceedings.mlr.press/v97/abu-el-haija19a.html},
}
@InProceedings{chen20v,
  title = 	 {Simple and Deep Graph Convolutional Networks},
  author =       {Chen, Ming and Wei, Zhewei and Huang, Zengfeng and Ding, Bolin and Li, Yaliang},
  booktitle = 	 {ICML},
  pages = 	 {1725--1735},
  year = 	 {2020},
  volume = 	 {119}, 
  url = 	 {https://proceedings.mlr.press/v119/chen20v.html},
}
@inproceedings{rahimi2018semi,
    title = "Semi-supervised User Geolocation via Graph Convolutional Networks",
    author = "Rahimi, Afshin  and
      Cohn, Trevor  and
      Baldwin, Timothy",
    booktitle = "Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    year = "2018",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/P18-1187",
    doi = "10.18653/v1/P18-1187",
    pages = "2009--2019",
}
@inproceedings{zilly2017recurrent,
  title={Recurrent highway networks},
  author={Zilly, Julian Georg and Srivastava, Rupesh Kumar and Koutn{\i}k, Jan and Schmidhuber, J{\"u}rgen},
  booktitle={International Conference on Machine Learning},
  pages={4189--4198},
  year={2017},
  organization={PMLR}
}
@inproceedings{he2016resnethu,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={CVPR},
  pages={770--778},
  year={2016}
}
@inproceedings{zhu2021interpreting,
  title={Interpreting and unifying graph neural networks with an optimization framework},
  author={Zhu, Meiqi and Wang, Xiao and Shi, Chuan and Ji, Houye and Cui, Peng},
  booktitle={The WWW},
  pages={1215--1226},
  year={2021}
}
@article{zhang2020implicitly,
  title={Implicitly defined layers in neural networks},
  author={Zhang, Qianggong and Gu, Yanyang and Mateusz, Michalkiewicz and Baktashmotlagh, Mahsa and Eriksson, Anders},
  journal={arXiv:2003.01822},
  year={2020}
}
@inproceedings{fu2022p,
  title={$ p $-Laplacian Based Graph Neural Networks},
  author={Fu, Guoji and Zhao, Peilin and Bian, Yatao},
  booktitle={International Conference on Machine Learning},
  pages={6878--6917},
  year={2022},
  organization={PMLR}
}
@article{bauschke2018breg,
  title={Regularizing with Bregman--Moreau envelopes},
  author={Bauschke, Heinz H and Dao, Minh N and Lindstrom, Scott B},
  journal={SIAM Journal on Optimization},
  volume={28},
  number={4},
  pages={3208--3228},
  year={2018},
  publisher={SIAM}
}
@inproceedings{fan2019graph,
  title={Graph neural networks for social recommendation},
  author={Fan, W. and Ma, Y. and Li, Q. and He, Y. and Zhao, E. and Tang, J. and Yin, D.},
  booktitle={The WWW},
  pages={417--426},
  year={2019}
}
@inproceedings{social1,
  title     = {Deep Reasoning with Knowledge Graph for Social Relationship Understanding},
  author    = {Wang, Zhouxia and Chen, Tianshui and Ren, Jimmy and Yu, Weihao and Cheng, Hui and Lin, Liang},
  booktitle = {IJCAI}, 
  pages     = {1021--1028},
  year      = {2018},
  doi       = {10.24963/ijcai.2018/142},
  url       = {https://doi.org/10.24963/ijcai.2018/142},
}
@article{wu2022graph,
  title={Graph neural networks in recommender systems: a survey},
  author={Shiwen Wu and Sun, Fei and Zhang, Wentao and Xie, Xu and Cui, Bin},
  journal={ACM Computing Surveys},
  volume={55},
  number={5},
  pages={1--37},
  year={2022},
  publisher={ACM New York, NY}
}
@inproceedings{bio1,
  title     = {Hybrid Approach of Relation Network and Localized Graph Convolutional Filtering for Breast Cancer Subtype Classification},
  author    = {Rhee, Sungmin and Seo, Seokjun and Kim, Sun},
  booktitle = {IJCAI}, 
  pages     = {3527--3534},
  year      = {2018},
  doi       = {10.24963/ijcai.2018/490},
  url       = {https://doi.org/10.24963/ijcai.2018/490},
}
@article{bio2,
  title={Graph-based deep learning for medical diagnosis and analysis: past, present and future},
  author={Ahmedt-Aristizabal, David and Armin, Mohammad Ali and Denman, Simon and Fookes, Clinton and Petersson, Lars},
  journal={Sensors},
  volume={21},
  number={14},
  pages={4758},
  year={2021},
  publisher={MDPI}
}
@inproceedings{zheng2020gman,
  title={Gman: A graph multi-attention network for traffic prediction},
  author={Zheng, Chuanpan and Fan, Xiaoliang and Wang, Cheng and Qi, Jianzhong},
  booktitle={AAAI},
  volume={34},
  number={01},
  pages={1234--1241},
  year={2020}
}
@inproceedings{trans1,
  title     = {Spatio-Temporal Graph Convolutional Networks: A Deep Learning Framework for Traffic Forecasting},
  author    = {Yu, Bing and Yin, Haoteng and Zhu, Zhanxing},
  booktitle = {IJCAI}, 
  pages     = {3634--3640},
  year      = {2018},
  doi       = {10.24963/ijcai.2018/505},
  url       = {https://doi.org/10.24963/ijcai.2018/505},
}
@inproceedings{ying2018graph,
  title={Graph convolutional neural networks for web-scale recommender systems},
  author={Ying, Rex and He, Ruining and Chen, Kaifeng and Eksombatchai, Pong and Hamilton, William L and Leskovec, Jure},
  booktitle={SIGKDD},
  pages={974--983},
  year={2018}
}
@article{zhou2020graph,
title = {Graph neural networks: A review of methods and applications},
journal = {AI Open},
volume = {1},
pages = {57-81},
year = {2020},
issn = {2666-6510},
doi = {https://doi.org/10.1016/j.aiopen.2021.01.001},
url = {https://www.sciencedirect.com/science/article/pii/S2666651021000012},
author = {Jie Zhou and Ganqu Cui and Shengding Hu and Zhengyan Zhang and Cheng Yang and Zhiyuan Liu and Lifeng Wang and Changcheng Li and Maosong Sun}
}
@article{dhillon2008matrix,
  title={Matrix nearness problems with Bregman divergences},
  author={Dhillon, Inderjit S and Tropp, Joel A},
  journal={SIAM Journal on Matrix Analysis and Applications},
  volume={29},
  number={4},
  pages={1120--1146},
  year={2008},
  publisher={SIAM}
}
@article{van2017forward,
  title={Forward-backward splitting with Bregman distances},
  author={Van Nguyen, Quang},
  journal={Vietnam Journal of Mathematics},
  volume={45},
  number={3},
  pages={519--539},
  year={2017},
  publisher={Springer}
}
@inproceedings{yan2022two,
  title={Two sides of the same coin: Heterophily and oversmoothing in graph convolutional neural networks},
  author={Yan, Yujun and Hashemi, Milad and Swersky, Kevin and Yang, Yaoqing and Koutra, Danai},
  booktitle={ICDM},
  pages={1287--1292},
  year={2022}, 
}
@article{combettes2020deep,
  title={Deep neural network structures solving variational inequalities},
  author={Combettes, Patrick L and Pesquet, Jean-Christophe},
  journal={Set-Valued and Variational Analysis},
  volume={28},
  pages={491--518},
  year={2020},
  publisher={Springer}
}
@article{hinton2012practical,
  title={A practical guide to training restricted Boltzmann machines},
  author={Hinton, Geoffrey E},
  journal={Neural Networks: Tricks of the Trade: Second Edition},
  pages={599--619},
  year={2012},
  publisher={Springer}
}
@inproceedings{chen2020measuring,
  title={Measuring and relieving the over-smoothing problem for graph neural networks from the topological view},
  author={Chen, Deli and Lin, Yankai and Li, Wei and Li, Peng and Zhou, Jie and Sun, Xu},
  booktitle={AAAI},
  volume={34},
  number={04},
  pages={3438--3445},
  year={2020}
}
@ARTICLE{CNN,
  author={Lecun, Y. and Bottou, L. and Bengio, Y. and Haffner, P.},
  journal={Proceedings of the IEEE}, 
  title={Gradient-based learning applied to document recognition}, 
  year={1998},
  volume={86},
  number={11},
  pages={2278-2324},
  doi={10.1109/5.726791}}
@inproceedings{li2018deeper,
  title={Deeper insights into graph convolutional networks for semi-supervised learning},
  author={Li, Qimai and Han, Zhichao and Wu, Xiao-Ming},
  booktitle={AAAI},
  volume={32},
  number={1},
  year={2018}
}
@article{wu2020comprehensive,
  title={A comprehensive survey on graph neural networks},
  author={Wu, Zonghan and Pan, Shirui and Chen, Fengwen and Long, Guodong and Zhang, Chengqi and Philip, S Yu},
  journal={IEEE TNNLS},
  volume={32},
  number={1},
  pages={4--24},
  year={2020},
  publisher={IEEE}
}
@article{meyes2019ablation,
  title={Ablation studies in artificial neural networks},
  author={Meyes, Richard and Lu, Melanie and de Puiseau, Constantin Waubert and Meisen, Tobias},
  journal={arXiv:1901.08644},
  year={2019}
}

